Prompt-based Visual Alignment for Zero-shot Policy Transfer

Overfitting in RL has become one of the main obstacles to applications in reinforcement learning(RL). Existing methods do not provide explicit semantic constrain for the feature extractor, hindering the agent from learning a unified cross-domain representation and resulting in performance degradation on unseen domains. Besides, abundant data from multiple domains are needed. To address these issues, in this work, we propose prompt-based visual alignment (PVA), a robust framework to mitigate the detrimental domain bias in the image for zero-shot policy transfer. Inspired that Visual-Language Model (VLM) can serve as a bridge to connect both text space and image space, we leverage the semantic information contained in a text sequence as an explicit constraint to train a visual aligner. Thus, the visual aligner can map images from multiple domains to a unified domain and achieve good generalization performance. To better depict semantic information, prompt tuning is applied to learn a sequence of learnable tokens. With explicit constraints of semantic information, PVA can learn unified cross-domain representation under limited access to cross-domain data and achieves great zero-shot generalization ability in unseen domains. We verify PVA on a vision-based autonomous driving task with CARLA simulator. Experiments show that the agent generalizes well on unseen domains under limited access to multi-domain data.

==> sec/4_experiment_zzh.tex <==

\section{Experiment}


%下面这段写到Environment setup里
\subsection{Setup}
In this section, we will deliver the details of the experiments to validate the agent's generalization ability in CARLA\cite{CARLA}. 
%rui：从下面开始，应该写对CARLA介绍的描述，因为可能reviewer根本不知道CARLA这个环境是什么样的。前两条原因关系不大，写在描述介绍里就行（第一条不要提CLIP，显得太刻意了），第三条可以写成我们选择CARLA的原因
\haihan{CARLA is an autonomous driving simulation engine which provides several maps including urban and suburban areas under different weather conditions and is used to test the adaptation performance of the autonomous driving agent. CARLA also provides generic sensors such as the RGB camera and Radar to generate multi-modal sensational input like the point cloud and BEV image. We use the RGB image captured by a camera fixed on the top of the vehicle to train an autonomous driving agent and validate its performance under different weather conditions, including shifts in illumination and rainfall.}
Various weather conditions are illustrated in Figure \ref{fig:diffweather}.


\begin{figure}[h]
\centering
\subfigure[ClearNoon]{
    \centering
    \includegraphics[width = 0.45 \columnwidth]{image/domainimages/ClearNoon.png}
}
\subfigure[HardRainNoon]{
    \centering
    \includegraphics[width = 0.45 \columnwidth]{image/domainimages/HardRainNoon.png}
}
\subfigure[\scalebox{0.9}{WetCloudySunset}]{
    \centering
    \includegraphics[width = 0.45\columnwidth]{image/domainimages/SoftRainSunset.png}
}
\subfigure[SoftRainSunset]{
\centering
    \includegraphics[width = 0.45\columnwidth]{image/domainimages/WetSunset.png}
}
\caption{Illustration of different domains. ClearNoon and HardRainNoon are used to tune the prompt and train the visual aligner. We validate the agent's performance on WetCloudySunset, ClearSunset, and SoftRainSunset, which do not appear in the training stage.}
\label{fig:diffweather}
\end{figure}
%rui：这个小标题不需要加吧，因为一共就只有一个环境
%\textbf{CARLA-based environment}
We build a reinforcement environment based on CARLA simulator.
The observation space consists of two parts: an image captured by the RGB camera fixed on the car and current velocity of the vehicle. Action space is a three-dimensional vector, two dimensions control the direction of the car and the other dimension corresponds with the car's acceleration. We have to control the vehicle from the start point to the destination. The environment will terminate when encountering one of the following termination conditions 
     1) The car has arrived at the destination.
     2) The car collapses with other objects. 
     3) The driving time exceeds the time limit.
     4) The car crosses the lane line.
% \end{itemize}
A negative punishment will be given if event 2), 3), and 4) occur and a positive reward will be given if the car arrive the destination before the time limit. We also want the vehicle to arrive at the destination as quickly as possible. For this reason, a constant negative reward will be given for every step. 
Each domain represents a specific type of weather, which is controlled by a set of parameters, including cloudiness, precipitation, sun altitude angle, and sun azimuth angle.



\subsection{Design of the model and details of training}
\textbf{Design of the Instance Prompt Learner $h_\phi$}: Instance Prompt Learner $h_\theta$ generates a sequence of learnable tokens directly from the image. $h_\theta$ consists of a ResNet19\cite{resnet} and $L_C$ MLP heads. The heads take the feature extracted by ResNet as the input and convert it into $L_C$ instance tokens. 

\textbf{Design of the Visual Aliger  $f_\theta$}: We apply UNet\cite{unet} as the visual aligner, UNet is composed of an encoder and a decoder and has a symmetric structure. The encoder extracts features from the raw image by a CNN layer with $3\times 3$ kernel. Pooling and Skip-connection are also applied in the encoder to reduce the dimension of features and fuse different layers. The decoder will recover the resolution from the feature map via upsampling. We constrain the UNet by aligning the visual representation of the transferred image with the tuned text presentation.

\textbf{Details of training:} With the help of the pretrained CLIP, A small dataset collected in various domains is applied in prompt tuning and visual alignment. In the experiment, we sample only 100 images from 2 different domains to extract semantic information and build the visual aligner. \haihan{The length of global, domain-specific, and instance prompts are 10, 5, and 10. We also applied different temperatures and learning rates to align the learnable prompts with the visual inputs. For general and domain-specific prompts, the temperature and learning rate are 0.5 and 0.0004. For instance-specific prompts, the temperature and learning rate are 0.1 and 0.00005. The prompt tuning takes 4 hours and visual alignment takes about 8 hours, both are conducted in A8000. }
%rui：重要的超参数还得写一写，现在好像没了。包括公式中的lambda值，prompt的长度，硬件条件用了什么卡训练的之类的
% \textbf{Hyper parameter}: The default hyperparams are illustrated in table \ref{tab:experimenthyper}. %这里用文字描述重要的超参数（不重要的不用写出来），不要列表

%写在实验结果部分，不是实验设置里

% We select a smaller temperature parameter
\subsection{Comparisons}

\ZZH{In this part, we evaluate our method from two perspectives. Firstly, we compare it with other state-of-the-art representation-based methods that utilize the experimental settings described in the original article. Subsequently, we reduce the training data of these methods to assess the generalization capability of our approach.}

\subsubsection{Comparison with existing methods}
We compared our method with representation-based methods, such as LUSR\cite{LUSR}, CURL\cite{CURL}, and DARLA\cite{darla}. These methods require data from various domains to pretrain a feature extractor and obtain a latent 
domain-shared representation of the visual inputs. The agent derives corresponding actions from the pretrained latent features. These methods aim to extract the domain-agnostic representation across different domains which can generalize to unseen domains. There are also several approaches that train an image-to-image translator, such as CycleGAN-RL\cite{cyclegan}, AdaIN\cite{instancestyletrans}, pix2pix\cite{pix2pix}, and UNIT4RL\cite{transferimagerl}. 
These approaches transform images from the source domain to the target domain.
% Similar to our method, image translation methods train visual mapping to translate the visual image from one domain to the target domain. % 采样动作中的电
% We separate the domains into two categories. The seen domains, including ClearNoon and HardRainNoon appear during the agent training. The agent has no access to any image on unseen domains. After visual alignment, we take the domain ClearNoon to train the RL agent and any other domain will align to ClearNoon.




The performance is illustrated in Table \ref{tab:performance}. Our method exceeds other approaches on unseen domains. Our method utilizes fewer images from multiple domains than other approaches illustrated in table \ref{tab:performance}. LUSR separates the latent representation into domain-agnostic and domain-specific parts and could generalize well on seen domains. DARLA utilizes $\beta-$VAE to learn a domain-agostic representation by adapting $\beta$. CURL use data augmentation and contrastive learning to learn the adaptable representation. We apply random crop and gray scale to create positive pairs. From the experiment results, we observe there exists performance degradation on unseen domain. For image-translation approaches, we find it could only handle the adaptation between two domains. Our approaches achieve higher generalization performance by alleviating the domain bias with less requirement to cross-domain images.
% We illustrated the visual representation generated by LUSR, DARLA, and CURL and can observe OOD phenomena on unseen domains.
% In Fig \ref{fig:latentdis}, we observe the latent distribution of images sampled from unseen domains does not match with those from seen domains.
In the baseline setting, we sampled 10000 images per domain to learn a cross-domain invariant representation or the image translator.
% PVA mitigates the requirement for cross-domain data.

\begin{table*}[h]
\centering
\begin{tabular}{cccccc}
    % \begin{tabular}{|l|>{\columncolor{blue!50}}c|>{\columncolor{red!50}}c|>{\columncolor{green!50}}c|>{\columncolor{green!50}}c|>{\columncolor{green!50}}c|}
    % \begin{tabular}{|l|ccccc|}
    \toprule
     \multirow{2}{*}{method} &\multicolumn{2}{c}{seen domains} & \multicolumn{3}{c}{unseen domains} \\
          \cmidrule(lr){2-3} \cmidrule(lr){4-6}
       & ClearNoon & HardRainNoon & ClearSunset & WetCloudySunset & SoftRainSunset \\ 
    \midrule
        LUSR & 1997.4 & 775.6 & 2079.0 & 582.8 & 533.8 \\ 
        % LUSR(ClearNoon only) & 1428.2 & 40.3 & 363.9 & 43.3 & 43.6 \\ 
        % PVA(learnable prompt, no base) & 1227.2 & 126.0 & 333.7 & 48.9 & 277.6 \\
        % PVA(fixed text,no base) & 1559.4 & 118.63 & 102.6 & 1141.6 & 856.72 \\ 
        DARLA & 1207.2 & 1257.4 & 450.3 & 162.5 & 1060.3 \\ 
        CURL & 1508.1 & 1308.4 & 801. & 998.5& 	1046.  \\ 
        UNIT4RL & 1636.4 & 322.7 & 298.1 & 239.8 & 383.5 \\
        CycleGAN & 1981.9 & 1528.8 & 277.0 & 637.4 & 657.1 \\ 
        pix2pix & 1821.7 & 520.5 & 157.5 & 420.9 & 662.9 \\ 
        AdaIN & 1829.6 & 285.8 & 499.9 & 101.7 & 245.3 \\ \midrule
        PVA(ours) & \textbf{2004.6} &\textbf{1825.9} & \textbf{2178.4} & \textbf{1775.65} & \textbf{1789.2} \\ 
        \bottomrule
    % \end{tabular}
\end{tabular}
\vspace{-0.5em}
    \caption{Domain Generalization Performance of PVA and other benchmarks in CARLA simulation task. ClearNoon and HardRainNoon is included in seen domains. The policy is trained in ClearNoon.}
    
    \label{tab:performance}
\end{table*}



% We also visualize the low-dimensional visual representation In Fig \ref{fig:latentdis}


We illustrate the inputs of RL agent, which is a latent representation compressed from the raw image. Data augmentation and representation-based methods suffer from distribution shifts between seen and unseen domains. Our approach mitigates differences between domains, which leads to better generalization performance by mapping various domains into an unified one.

% From the illustration of distributions, we observe other representation-based methods suffer from the distribution shift between seen domains and unseen domains, which indicates that the latent representation of images collected on unseen domains falls out of the distribution of the seen domain's representations. 
% Our method solves the problem by aligning the semantic information in the image with the tuned prompts, which leads to better generalization performance.


\begin{figure}[t]
\centering
\includegraphics[width=\columnwidth]{icml2024/image/distribution/figure4.pdf}
\caption{Visualization the distribution of latent embeddings of different domains, which serve as the input of the RL agent. Differerent colors is used to represent various domains respectively. We observe our approach alleviates the domain bias between domains, which makes the agent generalize under detrimental obervation difference.}
\label{fig:latentdis}
\end{figure}

\begin{table}[H]
    \centering
    % \begin{tabular}{cccccc}
   \begin{tabular}{ccc}
    % \begin{tabular}{|l|>{\columncolor{blue!50}}c|>{\columncolor{red!50}}c|>{\columncolor{green!50}}c|>{\columncolor{green!50}}c|>{\columncolor{green!50}}c|}
    % \begin{tabular}{|l|ccccc|}
    \toprule
     % \multirow{2}{*}{method} &\multicolumn{1}{c}{seen domains} & \multicolumn{1}{c}{unseen domains} \\
          % \cmidrule(lr){2-2} \cmidrule(lr){3-3}
      method & ClearNoon &  ClearSunset  \\ 
    \midrule
        CURL & 1227.4 & 199.5  \\ 
        AdaIN & 1420.8 & 313.9 \\ \midrule
        PVA(ours) & \textbf{2004.6} &\textbf{1825.9} \\ 
        \bottomrule
    % \end{tabular}
\end{tabular}
\vspace{-0.5em}
    % \begin{tabular}{c|c}
    %      &  \\
    %      & 
    % \end{tabular}
    \caption{Compared with other approaches with the same quantity of images.}
    \label{tab:same_amount}
\end{table}
% \vspace{-0.2cm}

% Then we train a RL agent by interacting with ClearNoon. The experiment results indicate these two baselines fail to generalize under limited access of data in various domains.


% \begin{figure}[h]
%     \centering
%     % \setlength{\belowcaptionskip}{-5mm}
%     % \begin{subfigure}{0.7\linewidth}
%     \includegraphics[width=0.7\columnwidth]{image/len.png}
%     % \end{subfigure}
%     \caption{size of $D_{semantic}$ influence on the agent performance.}
%     \label{fig:semsize}
% \end{figure} 
\subsubsection{Comparision with other baselines with the same number of images in training}

% 可以先讲一下实验目的，To verify the generalization ability of our method, we carry out the experiments comparing XXXX
The table \ref{tab:same_amount} shows the performance of baseline and our approach under the same amount of images used in training stage. 
% In LUSR, we sample 100 images from the domain HardRainNoon and mix with 10000 images in ClearNoon to extract the shared feature from the mixed dataset. 
\TODO{We applied 100 images from ClearNoon and HardRainNoon for all baselines illustrated in table \ref{tab:same_amount}. For CURL, we apply contrastive learning to learn a representation from these images.}
In AdaIN, the small dataset is used to train an image translator between two domains. 
% \ZZH{From the table, we can observe that our method have a higher XXX compared with CURL and AdaIN method. The reason is XXX}
The experiment results indicate these two baselines fail to generalize under limited access of data in various domains.

\subsection{Ablation studies}


% \textbf{The influence of the image number used for semantic extraction and visual alignment.} Here we propose a natural problem: will the performance degrade as the size of $D_{semntic}$ decreases? The experiment results are illustrated in Figure \ref{fig:semsize}
% \begin{figure}[h]
%     \centering
%     % \setlength{\belowcaptionskip}{-5mm}
%     % \begin{subfigure}{0.7\linewidth}
%     \includegraphics[width=0.7\columnwidth]{image/len.png}
%     % \end{subfigure}
%     \caption{size of $D_{semantic}$ influence on the agent performance.}
%     \label{fig:semsize}
% \end{figure} 
% The Figure illustrates that the model can not generalize with too less data, such as only 1 image per domain.

\textbf{Ablation study of different components of the prompt:} In this part, we conduct experiments to show the necessity of each component in our methods, including different parts in the prompts and replace the learnable prompt with a fixed natural language sequence, the results are illustrated in table \ref{tab:ablationstudy}. We find that both three components of prompts are beneficial for the adaptation performance. 
\TODO{According to the experiment result in table \ref{tab:ablationstudy}, the instance-conditional prompt has the most influential effects on the performance both on seen and unseen domains. We deduce that domain-specific prompts fail to depict instance-level information in our framework, which indicates the necessity of this part.}
% Domain-specific prompts have a crucial influence on the final result because the sequence contains the description of the domain's character. The global prompts give a universal depiction of the control problem. The experiment result indicates that removal of the global prompts will degrade performances in all domains.
%rui：后面对实验结果的分析和实验结论要写一写，文字里需要有实验结果的描述，比如，添加了A后结果提升了还是下降了，添加了B后结果提升了还是下降，这说明什么。

\textbf{Ablation study of loss function in $L_{total}$}. \haihan{In this part, we discuss the influence of different components in $L_{total}$ when training the visual aligner $f_\theta$. The result is illustrated in Table \ref{tab:ablationloss} .} \TODO{We observe $L_{feature}$ is crucial for overall performance and removal of $L_{feature}$ will cause performance degradation across all domains. $L_{global}$ and $L_{patch}$ have significant influence on the adaptation performance on new domains.}
% The feature loss $L_{feature}$ is widely applied in image translation to align the details between input images and output images, which is reasonable to keep the local details invariance. In contrast, $L_{global}$ is used to improve the agent's generalization ability because it contains semantic description which is domain-agnostic. 
% Our experiment indicates that $L_{feature}$ is crucial to generate images with good quality.


% \captionsetup[subfigure]{position=top}





%rui：实验结论要写成对自己有利的，比如说这几个loss都很重要都对结果提升有帮助
% \textbf{Comparison on prompt design}
% \textbf{Comparison on alignment}

% \subsection{Visualization}
% We visualize the aligned images in figure \ref{fig:visualaligner}. Our method generates high-quality images with similar appearance, which compensates for the domain differences caused by different lighting conditions.



% \resizebox{\linewidth}{!}{

% }

% \scalebox{0.95}{
\begin{table*}[ht]
\centering
\scalebox{0.95}{
\begin{tabular}{cccccc}
    \toprule
     \multirow{2}{*}{prompt} &\multicolumn{2}{c}{seen domains} & \multicolumn{3}{c}{unseen domains} \\
          \cmidrule(lr){2-3} \cmidrule(lr){4-6}
       & ClearNoon & HardRainNoon & ClearSunset & WetCloudySunset & SoftRainSunset \\ 
    \midrule
        % LUSR(full) & 1997.4 & 775.6 & 2079.0 & 582.8 & 533.8 \\ 
        % LUSR(ClearNoon only) & 1428.2 & 40.3 & 363.9 & 43.3 & 43.6 \\ 
        % PVA(learnable prompt, no base) & 1227.2 & 126.0 & 333.7 & 48.9 & 277.6 \\
        fixed sentence& 1559.4 & 118.63 & 102.6 & 1141.6 & 856.72 \\
        $\textcolor[rgb]{0,0,1}{[v_{s}^1]\cdots [v_{s}^{L_S}]}$$\textcolor[rgb]{1,0,0}{[v_C^1]\cdots [v_C^{L_C}]} $ & 1157.1 & 1120.7 & 716.0 & 1049.2 & 592.7  \\
        $\textcolor[rgb]{0,1,0}{[v_g^1]\cdots [v_g^{L_G}]}$$\textcolor[rgb]{1,0,0}{[v_C^1]\cdots [v_C^{L_C}]} $ & 1361.3 & 1425.48 & 852.6 & 1330.1 & 1055.2 \\
        $\textcolor[rgb]{0,1,0}{[v_g^1]\cdots [v_g^{L_G}]}$$\textcolor[rgb]{0,0,1}{[v_{s}^1]\cdots [v_{s}^{L_S}]}$ & 952.6 & 110.62 & 305.6 & 613.0 & 283.0 \\
        % DARLA & 1207.2 & 1257.4 & 450.3 & 162.5 & 1060.3 \\ 
        % UNIT4RL & 628.3 & 322.7 & 298.1 & 239.8 & 383.5 \\
        % CURL & 1508.1 & 1308.4 & 801. & 998.5& 	1046.  \\ 
        $\textcolor[rgb]{0,1,0}{[v_g^1]\cdots [v_g^{L_G}]}$$\textcolor[rgb]{0,0,1}{[v_{s}^1]\cdots [v_{s}^{L_S}]}$ $\textcolor[rgb]{1,0,0}{[v_C^1]\cdots [v_C^{L_C}]} $ & 2004.6 &{1825.9} & 2178.4 & {1775.7} & {1789.2} \\ 
        \bottomrule
\end{tabular}
}
\vspace{-0.5em}
    % \caption{Ablation study of the structure of prompt. This table illustrates the effects of different learnable parts as well as the fixed sentence. The fixed sentence is "Driving on the road on {xxx}" where xxx is the weather's name.}
    \caption{Ablation study of prompt structure. We observe the prompt tuning in stage 1 is effective in improving the generalization ability of the RL agent by replacing the tuned prompts with a fixed template.}
    \label{tab:ablationstudy}
% }
% \end{table*}
% % }
\vspace{1em}
% \begin{table*}[h]
% \subfigure[Ablation study of $L_{total}$]{
\begin{tabular}{cccccccc}
    % \begin{tabular}{|l|>{\columncolor{blue!50}}c|>{\columncolor{red!50}}c|>{\columncolor{green!50}}c|>{\columncolor{green!50}}c|>{\columncolor{green!50}}c|}
    % \begin{tabular}{|l|ccccc|}
    \toprule
     \multirow{2}{*}{method} & \multirow{2}{*}{$L_{global}$} & \multirow{2}{*}{$L_{patch}$} & \multirow{2}{*}{$L_{feature}$}  &\multicolumn{2}{c}{seen domains} & \multicolumn{2}{c}{unseen domains} \\
          \cmidrule(lr){5-6} \cmidrule(lr){7-8}
        & ~ & ~ & ~ & ClearNoon & HardRainNoon & ClearSunset & WetCloudySunset  \\ 
    \midrule
        with all loss function & $\checkmark$ & $\checkmark$ & $\checkmark$ & 2004.6 & 1825.9 & 2178.4 & 1775.6 \\ 
        without feature loss & $\checkmark$ & $\checkmark$ & $\times$ & 1175.0 & 147.7 & 111.4 & 83.9  \\ 
        without patch loss & $\checkmark$ & $\times$ & $\checkmark$ & 1420.8 & 1455.8 & 313.9 & 993.8  \\ 
        without global loss & $\times$ & $\checkmark$ & $\checkmark$ & 1533.4 & 1480.5 & 993.8 &  708.1 \\
        \bottomrule
    % \end{tabular}
\end{tabular}
\vspace{-0.5em}
    \caption{Ablation study of $L_{total}$. We observe $L_{feature}$ is crucial for adapting in HardRainNoon because it provide enough details during the transfer. $L_{global}$ and $L_{patch}$ are important for zero-shot adaptation on unseen domains.}
    \label{tab:ablationloss}
\end{table*}

\section{Conclusion}
We propose a visual alignment framework to enhance the generalization ability of reinforcement learning agents by training a visual aligner, which maps images from one domain to another domain. With the help of explicit semantic constraints, our approach achieves an excellent zero-shot domain adaptation performance.
Our methods utilize a sequence of learnable tokens to represent the semantic information in observations and tuned them with a pretrained VLM. Experiments conducted on a visual autonomous driving task shows our approach has a better generalization performance over unseen domains.
% With the help of the pretrained Visual Language Model, our method bridges the gap between text descriptions and image inputs, as well as alleviates the amount of data collected from various domains.
% \subsection{urther discussion: }
\section*{Impact Statements:}
Authors are required to include a statement of the potential broader impact of their work, including its ethical aspects and future societal consequences. This statement should be in a separate section at the end of the paper (co-located with Acknowledgements, before References), and does not count toward the paper page limit. In many cases, where the ethical impacts and expected societal implications are those that are well established when advancing the field of Machine Learning, substantial discussion is not required, and a simple statement such as:

“This paper presents work whose goal is to advance the field of Machine Learning. There are many potential societal consequences of our work, none which we feel must be specifically highlighted here.”

The above statement can be used verbatim in such cases, but we encourage authors to think about whether there is content which does warrant further discussion, as this statement will be apparent if the paper is later flagged for ethics review.
% The performance is illustrated in table \ref{tab:performance}. Our method exceeds other approaches on unseen domains. Our method utilize fewer images from multiple domains than other approaches illustrated in table \ref{tab:performance}. LUSR separates the latent representation into domain-agnostic and domain-specific parts and could generalize well on seen domains. However, there is severe performance degradation on unseen domains. We illustrated the visual representation generated by LUSR, DARLA, and CURL and can observe OOD phenomena on unseen domains. In Fig \ref{fig:latentdis}, we observe the latent distribution of images sampled from unseen domains does not match with those from seen domains. 
% $\textcolor[rgb]{0,1,0}{[v_g^1]\cdots [v_g^{L_G}]}$
% $\textcolor[rgb]{0,0,1}{[v_{s}^1]\cdots [v_{s}^{L_S}]}$ 
% $\textcolor[rgb]{1,0,0}{[v_C^1]\cdots [v_C^{L_C}]} $










